Multi-facet Universal Schema

Universal schema (USchema) assumes that two sentence patterns that share the same entity pairs are similar to each other. This assumption is widely adopted for solving various types of relation extraction (RE) tasks. Nevertheless, each sentence pattern could contain multiple facets, and not every facet is similar to all the facets of another sentence pattern co-occurring with the same entity pair. To address the violation of the USchema assumption, we propose multi-facet universal schema that uses a neural model to represent each sentence pattern as multiple facet embeddings and encourage one of these facet embeddings to be close to that of another sentence pattern if they co-occur with the same entity pair. In our experiments, we demonstrate that multi-facet embeddings significantly outperform their single-facet embedding counterpart, compositional universal schema (CUSchema) (Verga et al., 2016), in distantly supervised relation extraction tasks. Moreover, we can also use multiple embeddings to detect the entailment relation between two sentence patterns when no manual label is available.

==> EACL 2021/content/experiment.tex <==



We primarily compare our method with compositional universal schema (CUSchema)~\citep{verga2016multilingual} because CUSchema is one of the state-of-the-art RE methods in the small model regime (without using large pre-trained language models)~\cite{chang2016extracting,chaganty2017importance}.\footnote{We have not yet applied the multi-facet embeddings approach to the models that rely on a large pretrained language model (LM)~\cite{soares2019matching} due to computational and evaluation considerations. Computationally speaking, training state-of-the-art models requires intensive GPU resources. Besides, a smaller model size might be desired when we need to construct a knowledge base from a large corpus in real time.
%for the knowledge base construction tasks that need to process a large corpus in real time. 
Moreover, there is no existing pretrained LM in some domains~\cite{zhang2019openki}, and training the LM in a new domain from scratch requires even more GPU resources. 
%In practice, large training and testing corpus, but real time requirement -> smaller model size
%We do not have lots of GPU resources to perform the training as in state-of-the-art models such as \citet{soares2019matching}.

In terms of the evaluation consideration, our method is an improvement over CUSchema, so we want to compare it with CUSchema fairly. Furthermore, evaluating entailment between two full sentences is more difficult than between the sentence patterns, and we are not aware of a LM-based model that only considers the text between the entity pairs.}
%BERT is trained on the whole sentence, and we are not aware of the }
%whether BERT perform well in the sentence pattern setting is unknown.}
%easier on only the sentence pattern between the two entities.
%BERT is trained on the whole sentence, but 
%5. BERT requires long time to pretrain. 

In Section~\ref{sec:visual}, we visualize and analyze the facet embeddings. Next, we use distant-supervised RE tasks to evaluate our symmetric similarity measurement in Section~\ref{sec:RE_eval}, and detect entailment between sentence patterns to evaluate our asymmetric similarity measurement in Section~\ref{sec:entail_eval}. 
%In the visualization and entailment experiments, we test the model with the Transformer encoder that performs the best in the RE task.

%Introduce the three experiments
%~\ref{sec:entail_eval}

\begin{figure*}[t!]
\centering
\includegraphics[width=1\linewidth]{fig/Example_new.pdf}
\caption{Facet embedding visualization of \textbf{Ours (Single-Trans)} on the left and 
\textbf{Ours (Trans)} on the right. Dots are the facet embeddings outputted by our models and crosses are their nearby entity pair embeddings}
\label{fig:example}
\end{figure*}


\subsection{Embedding Visualization}
\label{sec:visual}
%($K=K_{KB}=1$) 
We visualize the embeddings of sentence patterns and a KB relation from the single embedding model and multi-facet embedding model that perform the best in the RE tasks (i.e., \textbf{Ours (Single-Trans)} and \textbf{Ours (Trans)} in Table~\ref{tb:TAC}). We project the facet embeddings to a 2-dimensional space using multidimensional scaling (MDS)~\cite{borg2005modern} and visualize the embeddings of one KB relation and three related sentence patterns in Figure~\ref{fig:example}. The three sentence patterns are selected from our validation set, so the model is not aware of the entity pairs that actually co-occur with the patterns during training. For each facet embedding, we show two among five of its closest entity pairs to visualize the meaning of the embedding space.\footnote{Notice that our training signal is sparse and noisy and the projection does not necessarily preserve the original distances, so the entity pairs with similar relations might be relatively far away from each other.}
%so it does not necessary able to distinguish the subtle difference between the relations of entity pairs.


%of 3 sentence patterns and 1 KB relation
%How do we get the visualization figure? nearby entity pair embeddings
%top 2 among top 5
%remove some entity pairs which are far away from its closest facet embedding after MDS projection
%random vector

In the single embedding model, the embedding of \textit{org:city\_of\_headquarter} is close to the embedding of \textit{(school, location)} while \textit{``\$ARG1 headoffice in \$ARG2''} is close to \textit{(company, location)} and \textit{``\$ARG1 headquarter in \$ARG2''}. 
%Explain the meaning of visualization
%in single embedding case 
%school location is closer to 
%organization location is closer to headoffice in

In the multi-facet embedding model, some embeddings of \textit{org:city\_of\_headquarter} are closer to \textit{(school, location)} and others are closer to \textit{(company, location)}. In addition to these entity pairs, \textit{``\$ARG1 headoffice in \$ARG2''} and \textit{``\$ARG1 headquarter in \$ARG2''} also co-occur with \textit{(people, location)} and \textit{(people/organization, year)}. Using the visualization of multi-facet embedding, we can understand which facets of \textit{org:city\_of\_headquarter} are similar or dissimilar to \textit{``\$ARG1 headoffice in \$ARG2''}, which cannot be done if all facets are averaged into a single embedding as in the traditional models.

The facet embeddings of \textit{``\$ARG1 is now at \$ARG2''} are close to \textit{(people, organization)} where the organization could be school, sports team, and company. Using multiple embeddings could avoid enforcing the closeness of these entity pairs with different relations. The results also indicate that our model can output reasonable cluster centers despite %via
learning from the sparse and noisy training data.
Finally, we can see that if a sentence pattern has fewer facets than $K$, our model learns to output some very similar facet embeddings, which makes the performance less sensitive to the setting of $K$.
%pattern
%the facet embeddings are often grouped together, which means our model learns to predict .
%Without  %such as \textit{(people, sports team)}, 

%different kinds of
%mostly \textit{(people, organization)}
%many different kinds 

%does not need to compress them very different entity pairs together


%Automatically determine the cluster number (KB relation)


%\textit{"\$ARG1 headoffice in \$ARG2"}

% (headoffice in)
 %by not averaging all embedding of co-occurring entity pair into a single point
%school location and organization location are close to both org:city\_of\_headquarter and headoffice in
%headoffice in also include
%similar in some aspects but dissimilar in some other


%equivalent to
%\textit{\$ARG1 headquarter in \$ARG2}




%related work section saying that lots of people solve various different settings but as far as we know, no one directly beats the compositional universal schema in their dataset

%The method achieves good performance on English~\cite{chaganty2017importance} and best performance on Spanish TAC 2016~\cite{chang2016extracting}


%\subsection{RE Datasets}





\subsection{Relation Extraction}
\label{sec:RE_eval}
We follow the same training data and testing protocol in compositional universal schema (CUSchema) \citep{verga2016multilingual}\footnote{\url{https://github.com/patverga/torch-relation-extraction}} to highlight the benefit of predicting multiple facet embeddings, and the relation extraction step in TAC KBP slot-filling tasks is used to compare the different models.
%make sure the improvement comes from .

\begin{table*}[t!]
\centering

\scalebox{0.9}{
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{|c|}{TAC 2012 (Validation)} & \multicolumn{3}{|c|}{TAC 2013} & \multicolumn{3}{|c|}{TAC 2014} \\ \cline{2-10}
& Prec & Recall & F1 & Prec & Recall & F1 & Prec & Recall & F1 \\ \hline
USchema* & \textbf{34.8} & 23.7 & 28.2 & \textbf{42.6} & 29.4 & 34.8 & \textbf{35.5} & 24.3 & 28.8 \\
CUSchema (LSTM)* &  27.0 & \textbf{32.7} & 29.6 & 39.6 & 32.2 & 35.5 & 32.9 & 27.3 & 29.8\\
%Ours (Single-LSTM) & 24.9 & 23.3 & 24.1 & 33.5 & 27.6 & 30.2 & 24.9 & 21.7 & 23.2  \\
Ours (Single-LSTM) & 25.7 & 21.7 & 23.5 & 30.4 & 26.3 & 28.2 & 22.1 & 20.5 & 21.3  \\
%Ours (Single-Trans) & 25.2 & 19.6 & 22.0 & 27.3 & 20.4 & 23.3 & 18.8 & 18.6 & 18.7  \\
%Ours (Single-LSTM) &  26.9 & 22.0 & 24.2 & 35.5 & 26.9 & 30.6 & 26.3 & 21.1 & 23.4 \\
Ours (Single-Trans) &  26.1 & 21.6 & 23.7 & 29.5 & 25.2 & 27.2 & 19.0 & 21.2 & 20.0 \\
Ours (LSTM) &  32.0 & 28.9 & 30.3 & 41.3 & \textbf{33.9} & 37.2 & 34.1 & \textbf{29.5} & \textbf{31.6} \\
%Ours (LSTM) &  32.9 & 28.5 & \textbf{30.5} & 39.6 & \textbf{33.3} & 36.2 & 35.3 & \textbf{29.7} & \textbf{32.2} \\
Ours (Trans) & 33.6 & 27.7 & \textbf{30.4} & 42.5 & 33.2 & \textbf{37.3} & 34.6 & 28.5 & 31.3 \\ \hline
USchema + CUSchema (LSTM)* & 29.3 & 32.8 & 30.9 & \textbf{41.9} & 34.4 & 37.7 & 29.3 & 34.1 &  31.5 \\
USchema + Ours (LSTM) & 29.2 & 33.7 & 31.3 & 38.1 & \textbf{38.9} & 38.5 & 31.5 & \textbf{34.4} & 32.9 \\ 
USchema + Ours (Trans) & \textbf{30.4} & \textbf{33.9} & \textbf{32.1} & 39.0 & 38.8 & \textbf{38.9} & \textbf{32.0} & 34.0 & \textbf{33.0} \\  \hline
\end{tabular}
}
\caption{Distantly supervised relation extraction using different versions of the universal schema. All numbers are \%. CUSchema refers to compositional universal schema. Trans is an abbreviation of Transformer. The best scores of the single models and ensemble models are highlighted. *The performance of TAC 2013 and 2014 are copied from \citet{verga2016multilingual}. }
\label{tb:TAC}
\end{table*}



%\noindent 
\textbf{Setup:} 
The training data for our RE models are prepared by distant supervision without requiring any manually labeled data.  The relations in Freebase \citep{bollacker2008freebase} are mapped to TAC relations (e.g., \textit{org:city\_of\_headquarter}) and the NER tagger and entity linker are run in a raw text corpus. Then, the training data is cleaned using the methods in \citet{roth2013survey}.
%The distant supervision assumption 

During testing, we are given a query containing the head entity and a query TAC relation in the slot-filling tasks, and the goal is to extract the tail entity from the candidate sentences. The NER tagger and query expansion are used to gather the candidate sentence patterns, and we compute the similarity scores from different models between the candidate sentence patterns and query relation. Finally, we compare the extracted second entity with the ground truth using exact string matching and report the precision, recall, and F1 scores.

Following \citet{verga2016multilingual}, we use TAC 2012 as our validation set to determine the threshold score for each TAC relation. Each model's hyperparameters are tuned separately using the validation set (TAC 2012) to ensure a fair comparison.
%(e.g., dropout rates) 
%to determine whether the candidates expressing the query relation.
%exact string matching

We compare the following methods: \\
\textbf{Ours (Trans)}:
Our method that measures the similarity between the sentence pattern~$\{\tilde{\underline{\vs}}_{i,k}\}$ and TAC relation~$\{\tilde{\underline{\vs}}_{j,m}\}$
using $Sim(\{\tilde{\underline{\vs}}_{i,k}\},\{\tilde{\underline{\vs}}_{j,m}\} )$ in \eqref{eq:sim_score}. Trans is an abbreviation of the Transformer encoder. We set $K=5$ and $K_{rel}=11$ based on the validation set.\\
\textbf{Ours (LSTM)}:
The same as Ours (Trans) except that we use bi-LSTM as our encoder instead. \\
\textbf{Ours (Single-*)}:
Our methods that use single facet embedding to represent each sentence pattern or KB relation. When setting $K=K_{rel}=1$, our decoder becomes the interleaving feedforward layers and cross-attention layers attending to the output embeddings of the encoder.\\
\textbf{CUSchema (LSTM)}: Compositional universal schema \citep{verga2016multilingual}. The method is similar to Ours (Single-LSTM) but uses a different loss function, neural architecture (no decoder), and hyperparameter search procedure. \\
\textbf{USchema}: Universal schema~\citep{riedel2013relation} estimates every sentence pattern embedding by factorizing the co-occurrence matrices (i.e., replacing the bi-LSTM in CUSchema with a look-up table). \\
\textbf{USchema + *}: \citet{verga2016multilingual} show that taking the maximal similarity between USchema and CUSchema model improves the F1. We also apply the same merging procedure to our model.
%We combine 



%as in \citet{verga2016multilingual}
%(\textbf{Ours (*)})
%and tune the hyperparameters (e.g., dropout rates) of our models. 

%multiple embedding models (\textbf{Ours (*)}) and single embedding models (\textbf{Ours (Single-*)}) 


%hyperparameter tuning. We do this separately on the multiple sentence pattern embedding and the single sentence pattern embedding.
%how to tune the relation threshold using validation set

%The label data are just used to tune the threshold of each relation and evaluate the performance.
%(except tuning the threshold). 


%Models to be compared

%During training, we map Freebase

%Our model does not require any label data during training.


%slot filling

%Use the same training data built in~\citet{verga2016multilingual}



%\noindent 
\textbf{Results:}
In Table~\ref{tb:TAC}, the proposed method \textbf{Ours (Trans)} significantly outperform \textbf{CUSchema (LSTM)} before and after combining with universal schema. As far as we know, our proposed multi-facet embedding is the first method that outperforms compositional universal schema using the same training signal in the distant-supervised RE benchmark they proposed.

Although the recall of \textbf{USchema} is low because it does not exploit the similarity between the patterns (e.g., \textit{``\$ARG1 happily married \$ARG2''} is similar to \textit{``\$ARG1 married \$ARG2''}), \textbf{USchema} has a high precision because it also won’t be misled by the similarity (e.g., \textit{``\$ARG1, and his wife \$ARG2''} expresses the \textit{spouse} relation but \textit{``\$ARG1, his wife, and \$ARG2''} does not)~\citep{verga2016multilingual}. Thus, combining \textbf{USchema} and \textbf{Ours (Trans)} leads to the best performance.

\textbf{Ours (Trans)} and \textbf{Ours (LSTM)} perform similarly. Furthermore, \textbf{Ours (LSTM)} performs much better than \textbf{Ours (Single-LSTM)}, which demonstrates the effectiveness of using multiple embeddings. 
Notice that multiple facet embeddings could improve the performance even after the training data have been cleaned. This indicates that our method is complementary to the noise removal methods in \citet{roth2013survey}.

%on top of the training data that have been 
%the training data have been cleaned and using . 


%using the methods in \cite{roth2013survey} and 
%, and our method could still improve the performance
%the improvement is . 
%\textbf{Ours (Single-LSTM)}
%, which  
%multiple embedding is effective

%\textbf{Our (LSTM)} performs much better than \textbf{Ours (Single-LSTM)}, which shows that the performance improvement majorly comes from the multiple embeddings.





%The improvement of LSTM is similar to the improvement of Transformer. This indicates that the improvement comes from the multiple embeddings representation.
%LSTM



%\textbf{Ours (Single-LSTM)} is worse than \textbf{CUSchema (LSTM)}. We suspect that it is due to the difference of our loss functions, and architectures, and hyperparameter search procedure.



% \begin{table}[t!]
% \centering
% \scalebox{0.6}{
% \begin{tabular}{|c|c|c|}
% \hline
% Specific Pattern & General Pattern & Label \\ \hline
% \$ARG1 , the president of the \$ARG2 & \$ARG1 , the leader of the \$ARG2 & E  \\
% \$ARG1 , chairman of the \$ARG2 & \$ARG1 , leader of the \$ARG2 & E  \\
% \$ARG1 's father , \$ARG2 & \$ARG1 's leader , \$ARG2  & N \\
% \$ARG1 worked with \$ARG2 & \$ARG1 deal with \$ARG2 & E  \\
% \$ARG1 had with \$ARG2 & \$ARG1 deal with \$ARG2 & N  \\
% \$ARG1 said \$ARG2 & \$ARG1 say the \$ARG2 & P  \\\hline

% \end{tabular}
% }
% \caption{}
% \label{tb:entail_examples}
% \end{table}




\begin{table*}[t!]
\centering
\scalebox{0.75}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Premise (Specific Pattern) & Hypothesis (General Pattern) & Label & Ours & CUSchema & Ours Diff &  Freq Diff  \\ \hline
\$ARG1 , the president of the \$ARG2 & \$ARG1 , the leader of the \$ARG2 & Entailment &  0.98 & 0.94 & + & +  \\
\$ARG1 's chairman , \$ARG2 & \$ARG1 's leader , \$ARG2 & Entailment &  0.95 & 0.87 & + & - \\
%\$ARG1 's father , \$ARG2 & \$ARG1 's leader , \$ARG2 & N & + & - &  0.04 & 0.52 \\
\$ARG1 's father , \$ARG2 & \$ARG1 's leader , \$ARG2 & Other &  0.08 & 0.52 & NA & NA  \\
\$ARG1 worked with \$ARG2 & \$ARG1 deal with \$ARG2 & Entailment &  0.92 & 0.83 & + & - \\
%\$ARG1 had with \$ARG2 & \$ARG1 deal with \$ARG2 & N & - & + &  0.44 & 0.88 \\
\$ARG1 had with \$ARG2 & \$ARG1 deal with \$ARG2 & Other &  0.96 & 0.88 & NA & NA \\
%\$ARG1 said the \$ARG2 & \$ARG1 say the \$ARG2 & P & + & - &  0.42 & 0.92 \\\hline
\$ARG1 said the \$ARG2 & \$ARG1 say the \$ARG2 & Paraphrase & 0.93 & 0.92 & NA & NA \\\hline

\end{tabular}
}
\caption{Example of sentence pattern pairs, its label, and our predictions in our entailment experiment. \textbf{Ours} and \textbf{Ours Diff} are the predictions from \textbf{Ours (Trans)}. \textbf{Freq Diff} is the frequency difference baseline. }
%E, O, and P means entailment, other, and paraphrase, respectively.
\label{tb:entail_examples}
\end{table*}



%Direction 
\subsection{Entailment Detection}
\label{sec:entail_eval}

Entailment is a common and fundamental relation between two sentence patterns. Some examples could be seen in Table~\ref{tb:entail_examples}. Unsupervised hypernym detection (i.e., entailment at the word level) is extensively studied~\cite{shwartz2017hypernyms}, but we are not aware of any previous work on unsupervised entailment detection at the sentence level, nor any existing entailment dataset between sentence patterns. Thus, we create one. %manually. %with the help of WordNet.

%Table~\ref{tb:entail_examples}

%It is more 
%We are not aware of any entailment dataset between sentence patterns, so we create one. %a small one

%\noindent 
\textbf{Dataset Creation:}
%\subsubsection{}  
We use WordNet~\citep{miller1998wordnet} to discover the entailment candidates of sentence pattern pairs and manually label the candidates. For each sentence pattern in the training data of \citet{verga2016multilingual}, we replace one word at a time with its hypernym based on the WordNet hierarchy. The two sentence patterns before and after replacement form an entailment candidate. 

We label 1,500 pairs of the most popular sentence pattern, which co-occurs with the highest number of unique entity pairs. Each candidate could be labeled as entailment, paraphrase, or other. Finally, around 20\% of the candidates are randomly chosen to form the validation set, and the rest are in the test set. More details of the dataset creation process could be seen in \refAppendixEntail
%we split the dataset into validation set and testing set with .

%that co-occur with the most unique entity pairs.
%most popular 
%classify the candidates into entailment, paraphrase, or other.

In this dataset, only 22\% and 10\% of candidates are labeled as entailment and paraphrase, respectively. This suggests that entailment relation between two sentence patterns is hard to be inferred by only the hypernym relation (i.e., entailment relation at the word level) in WordNet.
%in the sentence level is significantly different from the 

%how many entailment
%22\%
%10\%
%the rest of them are neutral

%wordnet baseline would be poor -> sentence level can do more than word level
%we usually cannot determine the direction based on the length of the sentence

%validation set size
%validation set to tune the hyperparameters

%hypernym replacement

%sort based on their min frequency
%how do we label them
%1500

%using direction detection micro accuracy

%\noindent 
\textbf{Setup:}
We evaluate entailment detection using the typical setup and metrics in hypernym detection \citep{shwartz2017hypernyms}. Negative examples include the candidates labeled as paraphrases and others. We compare the average precision of different methods (i.e., AUC in the precision-recall curve)~\citep{hastie2009elements}. In addition, we predict the direction of entailment relation in each pair (i.e., which pattern is the premise) and report the accuracy. Many hypotheses have the same hypernyms
%Some general hypernyms often appear in the hypothesis 
such as the \textit{leader} in Table~\ref{tb:entail_examples}, so we also report the macro accuracy of direction detection averaged across every hypernym in the hypotheses.

%\subsubsection{Setup}
%(the best one is the one we use in )

%we usually cannot predict the direction based on the length of the sentence pattern.
%synonym is negative examples as in common hypernym detection method \cite{shwartz2017hypernyms}


%set up the entailment detection task similar to 
%common 
%the paraphrases are negative examples\footnote{as in common hypernym detection dataset \cite{shwartz2017hypernyms}}

%direction detection

%explain micro and macro meaning using the table
%Table~\ref{tb:entail_examples}

The task is challenging because all the candidates have a word-level entailment relation if their compositional meaning is ignored. Furthermore, we cannot infer the entailment direction based on the tendency that longer sentence patterns tend to be more specific because most of the candidate pairs in this dataset have the same length.

%, and the length of two sentence patterns are usually the same.
%explain our method

As described in Section~\ref{sec:scoring}, our models detect the direction by computing 
\textbf{Ours Diff} as $Asym(\{\tilde{\underline{\vs}}_{i,k}\},\{\tilde{\underline{\vs}}_{j,m}\} ) - Asym(\{\tilde{\underline{\vs}}_{j,m}\}, \{\tilde{\underline{\vs}}_{i,k}\} )$ and
predict the $i$th sentence pattern to be 
premise if \textbf{Ours Diff} $> 0$. When performing entailment classification, we use as the asymmetric similarity scores $Asym(\{\tilde{\underline{\vs}}_{i,k}\},\{\tilde{\underline{\vs}}_{j,m}\} )$. We report the performance of \textbf{Ours (Trans)}, which is the same best model in the RE experiment.

%In direction detection, 

In entailment classification, we compare the results with cosine similarity from \textbf{Ours (Single-Trans)} and \textbf{CUschema}. 
We also test the frequency difference, which is a strong baseline in hypernym direction detection~\cite{chang2018distributional}. \textbf{Freq Diff} = Freq($S_j$) - Freq($S_i$) where Freq($S_i$) is the number of unique entity pairs co-occurred with the $i$th sentence pattern. The baseline predicts $S_i$ to be premise if \textbf{Freq Diff} $> 0$ because more general sentence patterns should co-occur with more entity pairs. As a reference, we also report the performance of random scores.
%difference of unique co-occurred entity pair numbers between sentence patterns because 

%CUschema uses cosine similarity to retrieve the entailment
%explain frequency baselines

%random

%that perform the best in relation extraction task.
%tends to be 

%When performing direction detection, our models use the sign of $Asym(\{\tilde{\underline{\vs}}_{i,k}\},\{\tilde{\underline{\vs}}_{j,m}\} ) - Asym(\{\tilde{\underline{\vs}}_{j,m}\}, \{\tilde{\underline{\vs}}_{i,k}\} )$

%premise
%$\{\tilde{\underline{\vs}}_{i,k}\}$
%hypothesis
%$\{\tilde{\underline{\vs}}_{j,k}\}$

%\eqref{eq:asym_score}
%Ours Diff

\begin{table}[t!]
\centering

\scalebox{0.8}{
\begin{tabular}{|c|c|cc|}
\hline
\multirow{2}{*}{Method} & Classification & \multicolumn{2}{|c|}{Direction Detection}  \\ \cline{2-4}
& AP@all & Micro Acc & Macro Acc \\ \hline
Random & 21.9 & 50.0 & 50.0\\
Freq Diff & 21.4 & 54.5 & 47.3 \\
CUSchema & 31.2 & 50.0 & 50.0\\
Ours (Single) & 23.6 & 50.0 & 50.0 \\
Ours& \textbf{37.8} & \textbf{63.1} & \textbf{55.4} \\ \hline
\end{tabular}
}
\caption{Comparison of entailment detection methods. AP and Acc are average precision and accuracy, respectively. All numbers are \%. Our methods use a Transformer as their encoder. %Ours and Ours (Single) refers to } 
}
\label{tb:entailment}
\end{table}

%\noindent 
\textbf{Results:}
%\subsubsection{Results}
The quantitative and qualitative comparison are presented in Table~\ref{tb:entailment} and Table~\ref{tb:entail_examples}, respectively. Our model that uses multi-facet embeddings significantly outperforms the other baselines. We hypothesize that a major reason is that the sentence patterns with an entailment relation are often similar in some but not all of the facets, and our asymmetric similarity measurement is better at capturing the facet overlapping.

%, which demonstrate the effectiveness of our asymmetric similarity mea
%better at discover entailment because one of the facets close to all other facets might give us the high similarity score

==> EACL 2021/content/experiment_details.tex <==

The details of preparing the entailment dataset are included in Section~\ref{sec:entailment_detail}, and the details of our experiment setup are included in Section~\ref{sec:setup_detail}. We present the results of our ablation studies in Section~\ref{sec:ablation_detail}.

\subsection{Entailment Dataset Creation}
\label{sec:entailment_detail}
When finding the entailment candidates using WordNet, we iterate over all the words in every sentence pattern. For each word, we retrieve all of its senses/synsets and the possible hypernym synsets. Finally, we replace the word with every lemma of each hypernym synset. After the replacement, if the sentence pattern appears in our training data, we pair the sentence patterns before and after replacement as a candidate.


%discover senses of each word using synsets
%find hypernym of each sense
%find all lemma of each hypernym

%how the entailment dataset is created (says that we cannot rely on the sentence length to distinguish the direction)

%For the sentence pattern, 

Our goal is to find entailment rather than paraphrase relation, so we exclude the candidates where the replaced word is both the hypernym and hyponym of the replacing word.
To measure each sentence pattern's popularity, we compute the number of unique entity pairs co-occurring with the sentence pattern as the pattern frequency and take the minimum of the frequency between the two sentence patterns in a candidate as the candidate frequency. 
For each hypothesis, we only consider the top 6 premise candidates with the highest frequencies to diversify the hypotheses in our dataset. The hypothesis popularity score is the average candidate frequencies across its top 6 premises.

Before labeling, we sort the hypotheses based on their popularity scores and label the most popular 1,500 candidates (with the highest minimal frequencies). The labeling is done by a PhD student who has RE research experiences because we hypothesize that it is hard to clearly explain the task to crowdsourcing workers. After the dataset is built, we separate the validation set and test set such that all hypernyms in the test hypotheses are unseen in the validation set.

%according to the hypernyms in the hypothesis. Thus, all the 

%validation split

%We hypothesize that it is hard to explain the task clearly to crowdsourcing workers, so the label is done by a PhD student who has research experience on relation extraction.


%sort based on their min frequency
%the both entailment in both direction cases

%truncate

%avoid too many premises come from the same hypothesis, top 6 premises for each hypothesis
%sort based on their minimal frequency
%compute macro easier and more stable


%and start from labeling the candidates 


%
%The label is done by a PhD student
%\section{More Experiments}

%Spanish
%\cite{chang2016extracting}
%2016 evaluation is different from 2012 evaluation (different ways of tuning threshold, different ways of treating unannotated samples because Lots of examples are contributed by Pat’s model. )
\subsection{Experiment Setup Details}
\label{sec:setup_detail}

In our visualization experiment, we filter out a few entity pairs that co-occur with less than 5 sentence patterns or become far away from its closest facet embedding after the projection. To prevent the facet embeddings from overlapping, we add a small random vector to each facet embedding.

In the co-occurrence matrix, we use 5\% of the unique sentence patterns as our validation set. All the sentence patterns in the validation set are unseen in the training set. We use the validation set to tune the number of epochs during training.
%training testing split
%unique sentence pattern
%5\%
%determine the best model before the maximal epoch number

We use coordinate descent to search the hyperparameters that result in the best F1 score in TAC 2012 during training (i.e., change one hyperparameter at a time). Compared with the grid search used in \textbf{CUSchema}, this tuning method is less computationally expensive and less likely to overfit the validation data. 

We first optimize the hyperparameters in \textbf{Ours (Trans)}. The search ranges are $\gamma=[0.1, 0.2, 0.3]$, $K=[1, 2, 3, 4, 5, 6, 11]$, $K_{rel}=[1, 8, 9, 10, 11, 12, 13, 14, 15]$, encoder dropout rate $=[0.25, 0.3, 0.35]$, learning rate for updating $\bm{H}=[1, 0.1, 0.01]$ and maximal epoch number $=[15, 20, 25, 30, 50]$. Our best Transformer model \textbf{Ours (Trans)} used $\gamma=0.2$, $K=5$, $K_{rel}=11$, encoder dropout rate $= 0.3$, learning rate for updating $\bm{H}=0.1$ and maximal number of epochs = 50. Then, we start from these best hyperparameters for \textbf{Ours (Trans)} and tune only encoder dropout rate $=[0.25, 0.3, 0.35]$, and maximal epoch number $=[15, 20, 25, 30, 50]$ for \textbf{Ours (LSTM)}. The best performing LSTM model used maximal 30 epochs while all other hyperparameters are found to be the same as the best Transformer model. Finally, we fix $K=K_{rel}=1$ and tune the hyperparameters using the same range as above, for \textbf{Ours (Single-Trans)} and \textbf{Ours (Single-LSTM)}. 

%Autoencoder weight


%To save the computational resources

%for hyperparameter optimization
%CUSchema uses grid search

%Hyperparameter range

\subsection{Ablation Study}
\label{sec:ablation_detail}

In Table~\ref{tb:TAC_ablation}, we justify using the autoencoder loss and using different facet numbers for sentence patterns ($K$) and for KB relations ($K_{rel}$). We can see that performance drops if we remove these techniques from our models using a Transformer. 


%design 
%test what would happen if we remove the autoencoder regularization and setting the number of facets for sentence patterns ($K$) the same as the number of facets for KB relations ($K_{rel}$)



\begin{table}[t!]
\centering

\scalebox{0.9}{
\begin{tabular}{|c|c|c|c|}
\hline
Method & 2012 & 2013 & 2014 \\ \hline
Ours & \textbf{30.4} & \textbf{37.3} & \textbf{31.3} \\ 
Ours ($K=K_{rel}=11$) & 29.9 & 36.1 & 29.8 \\
Ours (No autoencoder) & 27.5 & 33.5 & 30.2 \\ \hline
\end{tabular}
}
\caption{Ablation study on TAC datasets. All numbers are F1 (\%). All models use the Transformer encoder. }
\label{tb:TAC_ablation}
\end{table}


==> EACL 2021/content/introduction.tex <==



Relation extraction (RE) is a crucial step in automatic knowledge base construction (AKBC). A major challenge of RE is that the frequency of relations in the real world is a long-tail distribution but collecting sufficient human annotations for every relation is infeasible~\citep{han2020more}. 
%there are many long-tail 

%a tuple \textit{(Angelina Jolie, spouse, Brad Pitt)} in a knowledge base and . 
%Then, we assume the sentence pattern \textit{"\$ARG1, the partner of fellow \$ARG2"} is similar to \textit{(\$ARG1, spouse, \$ARG2)}, so 

Distant supervision is proposed to alleviate the issue~\citep{mintz2009distant}. Distant supervision assumes that a sentence pattern expresses a relation if the sentence pattern
co-occurs with an entity pair and the entity pair has the relation. For example, we assume the sentence pattern \textit{``\$ARG1, the partner of fellow \$ARG2''} is likely to express the spouse relation if we observe a text clip \textit{``... Angelina Jolie, the partner of fellow Brad Pitt ...''} in our training corpus and a knowledge base tells us that \textit{Angelina Jolie} and \textit{Brad Pitt} has the spouse relation.
Accordingly, we can infer that another entity pair is likely to have the spouse relation if we observe the text \textit{``, the partner of fellow''} between them in a new corpus.

\begin{figure}[t!]
\centering
\includegraphics[width=1\linewidth]{fig/first_page.pdf}
\caption{Comparison between the multi-facet and compositional universal schema. In our training loss, we encourage one of the facet embeddings from a sentence pattern to be similar to its co-occurred entity pair.}
%if they co-occur with the same entity pair.}
\label{fig:first_page}
\end{figure}

%sentence pattern

Universal schema~\citep{riedel2013relation} extends this assumption by treating every sentence pattern as a relation, which means we assume that sentence patterns or relations in a knowledge base are similar if they co-occur with the same entity pair. For example, we assume \textit{``\$ARG1, the partner of fellow \$ARG2''} and \textit{``\$ARG1, the wife of fellow \$ARG2''} are similar if they both co-occur with \textit{(Kristen Bell, Dax Shepard)}. Consequently, we can infer that \textit{``\$ARG1, the wife of fellow \$ARG2''} also implies spouse relation as \textit{``\$ARG1, the partner of fellow \$ARG2''} even if the knowledge base does not record the spouse relation between \textit{Kristen Bell} and \textit{Dax Shepard}.
%the knowledge base does not record the spouse relation of \textit{(Kristen Bell, Dax Shepard)}.

Compositional universal schema~\citep{verga2016multilingual} realizes the idea by using a LSTM~\citep{hochreiter1997long} to encode each sentence pattern into an embedding and encouraging the embedding to be similar to the embedding of the co-occurred entity pair. 
As in the lower part of Figure~\ref{fig:first_page}, the model makes the embeddings of two sentence patterns similar if they co-occur with the same entity pair. \citet{soares2019matching} rely on a similar assumption and achieve state-of-the-art results on supervised RE tasks by replacing the LSTM with a large pre-trained language model.

%embedding of all entity pairs that co-occur with the sentence pattern. 

\begin{figure*}[t!]
\centering
\includegraphics[width=1\linewidth]{fig/architecture.pdf}
\caption{An illustration of the proposed method. The training signal comes from the co-occurrence matrices of the KB and training text corpus on the right. On the lower left, we visualize our neural encoder, which captures the compositional meaning of tokens in the sentence pattern, and our neural decoder, which models the dependency among multiple facet embeddings. When a sentence pattern co-occurs with an entity pair, the training loss minimizes the distance between the entity pair embedding and the closest facet embedding of the sentence pattern (e.g., 0.2 between $s_{i,2}$ and $e_{1}$). Trainable parameters in our model are highlighted using red borders.
On the upper left, we visualize the embedding space to establish the connection between our method and clustering. 
%says somewhere that the columns and rows are reversed
}
\label{fig:architecture}
\end{figure*}

The variants of universal schema have many different applications, including multilingual RE~\cite{verga2016multilingual}, knowledge base construction~\cite{toutanova2015representing,verga2017generalizing}, question answering~\cite{das2017question}, document-level RE~\cite{verga2018simultaneously}, N-ary RE~\cite{akimoto2019cross}, open information extraction~\cite{zhang2019openki}, and unsupervised relation discovery~\cite{percha2018global}. 
%elsahar2017unsupervised
%liang2019relation

Nevertheless, one sentence pattern could contain multiple facets, and each facet could imply a different relation. In Figure~\ref{fig:first_page}, \textit{``\$ARG1, the partner of fellow \$ARG2''} could imply the entity pair has the spouse relation, the co-worker relation, or both. \textit{``\$ARG1 moved in with \$ARG2''} could imply the spouse relation, the parent relation, ..., etc. If we squeeze the facets of a sentence pattern into a single embedding, the embedding is more likely to be affected by the irrelevant facets from other patterns co-occurred with the same entity pair (e.g., \textit{``\$ARG1 moved in with \$ARG2''} might incorrectly imply the co-worker relation).
%let the irrelevant facets

Another limitation is that single embedding representation can only provide symmetric similarity measurement between two sentence patterns. Thus, an open research challenge is to predict the entailment direction of two sentence patterns only based on their co-occurring entity pair information. 

To overcome the challenges, we propose multi-facet universal schema, where we assume that two sentence patterns share a similar facet if they co-occur with the same entity pair. As in Figure~\ref{fig:first_page}, we use a neural encoder and decoder to predict multiple facet embeddings of each sentence pattern and encourage one of the facet embeddings to be similar to the entity pair embedding. As a result, the facets that are irrelevant to the relation between the entity pairs are less likely to affect the embeddings of entity pairs and other related sentence patterns. For example, the parent facet of \textit{``\$ARG1 moved in with \$ARG2''} could be excluded when updating the embeddings of \textit{(Angelina Jolie, Brad Pitt)}.

In our experiments, we first compare the multi-facet embeddings with the single-facet embedding in distantly supervised RE tasks. The results demonstrate that multiple facet embeddings significantly improve the similarity measurement between the sentence patterns and knowledge base relations. Besides RE, we also apply multi-facet embeddings to unsupervised entailment detection tasks. In a newly collected dataset, we show that multi-facet universal schema significantly outperforms the other unsupervised baselines.


%The multi-facet embedding opens the possibility of 
%To evaluate the direction

%our goal is to test whether using multiple embeddings to represent every sentence pattern is better than 
%we compare 
%We verify the effectiveness of our 
%experiment


%examples
%clustering center

%to represent an sentence pattern
%explain how neural encoder and decoder could solve the issue

%share one of facets assumption

%won't be affected by other
%One limitation of universal schema is that 
%one sentence pattern or KB relation should have multiple facets
%live in 

%explain the limitation of universal schema assumption (loss of information, will be affected more easily by noise, can only measure the similarity)

%when a sentence pattern expresses or implies multiple relations
%e.g., partner and coworker
%move in
%the very different relations need to be pull closer


%explicitly mention that we want to answer scientific question: 
%Whether multiple embedding could be more effective than single embedding

%Experiment design
%Does multiple embedding better than single embedding?
%Is it possible to learn entailment without supervision?



%explain the application of universal schema

%including matching the blank paper uses this assumption


%Relation extraction 
%RE long tail challenge (relation discovery)
%hard to collect label data for all different kinds of relations
%distant supervision

%between knowledge base and sentence
%It can be also between sentences

%If two sentences share the same entity pairs, they are similar and more likely to express the same relation

%Explain what universal schema is using sentence similarity perspective



%multiple modes are required for two reasons
%1. multiple relations (and his wife and coworker), could co-occur with multiple KB relation -> more specific patterns should have more diverse entity pairs -> and (more often)
%2. multiple possible entity pairs (and her partner, move in with) -> this also coorelates multiple relations -> more general patterns should have more diverse entity pairs -> or


==> EACL 2021/content/method.tex <==



Our method is illustrated in Figure~\ref{fig:architecture}. In Section~\ref{sec:background}, we first provide our problem setup: We are given a knowledge base (KB) and a text corpus during training. Our goal is to extract relations by measuring the similarity between KB relations and an (unseen) sentence pattern or to detect entailment between two sentence patterns. In Section~\ref{sec:neural}, we introduce our neural model, which predicts multi-facet embeddings of each sentence pattern. Next, in Section~\ref{sec:obj}, we describe our objective function, which encourages the embeddings of co-occurred entity pairs to be close to the embeddings of their closest pattern facets. Finally, in Section~\ref{sec:cluster}, we explain that multi-facet embeddings could be viewed as the cluster centers of possibly co-occurred entity pairs, and in Section~\ref{sec:scoring}, we provide our scoring functions for distantly supervised RE and unsupervised entailment tasks.

%~\citep{chang2016extracting}

\subsection{Background and Problem Setup}
\label{sec:background}
Our RE problem setup is the same as compositional universal schema~\citep{verga2016multilingual}. First, we run named entity recognition (NER) and entity linking on a raw corpus. After identifying the entity pairs in each sentence, we prepare a co-occurrence matrix as in Figure~\ref{fig:architecture}. Similarly, we represent the KB relations between entity pairs as a co-occurrence matrix and merge the matrices from the KB and the training corpus. The merged matrix has $y_{i,j} = 1$ if the $i$th sentence pair or KB relation co-occurs with the $j$th entity pair and $y_{i,j} = 0$ otherwise. 

%in the knowledge base (KB)
%the entities have been extracted and linked in the training corpus

During testing, we use NER to extract an entity pair and the sentence pattern, which might not have been seen in the training corpus. Next, we extract relations by computing the similarity between the sentence pattern embeddings and the embeddings of the applicable KB relations. Besides RE, we also detect the entailment between two sentence patterns by comparing their embeddings.

%Our setup is the same except we also want to 
%unseen during testing time
%a $N \times J$ 
%matrix $\bm{Y^{KB}}=[y^{KB}_{n,j}]_{n,j}$, where $y^{KB}_{n,j} = 1$ if the $j$th entity pair has the $n$th relation in KB and $y^{KB}_{i,j} = 0$ otherwise.

%$S=\cup_{i=1}^I \{S_i\}$ and a $I \times J$ matrix $\bm{Y^C}=[y^C_{i,j}]_{i,j}$, where $S_i$ is the $i$th sentence pattern and $y^C_{i,j} = 1$ if the $i$th sentence pair co-occur with the $j$th entity pair and $y^C_{i,j} = 0$ otherwise.

%$\mathbf{Y^{C}}$





\subsection{Neural Encoder and Decoder}
\label{sec:neural}

We use a neural model to predict $K$ facet embeddings of each sentence pattern. The goal is similar to \citet{NSD}, which predict a fixed number of embeddings of a sentence, so we adopt their neural model as shown in Figure~\ref{fig:architecture}.

%or a phrase
%Our goal is to use  

For the $i$th sentence pattern $S_{i}$, we append an \lessgreat{eos} to its end and use a 3-layer Transformer~\cite{vaswani2017attention} encoder $TE$ to model the compositional meaning of the input word sequence: 
%The word sequence is fed into a , and 
%\begin{align}
$\underline{\vu}_{i,1} ... \underline{\vu}_{i,|S_i|} \underline{\vu}_{i,\text{\lessgreat{eos}}} = 
TE( S_{i} \text{\lessgreat{eos}} ), $
where $\underline{\vu}_{i,l}$ is an embedding contextualized by the encoder. In the experiment, we also replace the Transformer with a bidirectional LSTM (bi-LSTM) to show that the improvement of multi-facet embeddings is independent of the encoder choice.

%Notice that the Transformers could be replaced by any encoder and we try LSTM. 
The embedding $\underline{\vu}_{i,\text{\lessgreat{eos}}}$ represents the whole sentence pattern; we use $K$ different linear layers $L^d_k$ to transform the embedding into the inputs of our decoder:
$\underline{\vb}_{i,k} = L^d_k(\underline{\vu}_{i,\text{\lessgreat{eos}}})$.

%To diversify the cluster centers, we first let the embedding $\underline{\vu}_{i,\text{\lessgreat{eos}}}$ 
%pass through different linear layers $L^d_k$ for different cluster centers:
%$\underline{\vb}_{i,k} = L^d_k(\underline{\vu}_{i,\text{\lessgreat{eos}}})$, 

The facets in a sentence pattern often have some dependency. For example, the patterns that express the partnership between two people might also express the collaboration relation between two companies. To leverage the dependency, we use another 3-layer Transformer as our decoder $TD$. Besides the self-attention, we allow the hidden states in the decoder to query the contextualized word embeddings $\underline{\vu}_{i,l}$ from the encoder~\cite{vaswani2017attention} and output the embeddings corresponding to the different facets $\underline{\vd}_{i,k}$: $\underline{\vd}_{i,1} ... \underline{\vd}_{i,K} = TD(\underline{\vb}_{i,1} ..., \underline{\vb}_{i,K}, \underline{\vu}_{i,1} ... \underline{\vu}_{i,\text{\lessgreat{eos}}}).$ Notice that we do not use autoregressive decoding as in~\citet{vaswani2017attention}, so our decoder could also be viewed as another encoder with attention to the output of the encoder $TE$. Finally, to convert the hidden state size to the entity embedding size, we let the outputs of decoder go through another linear layer $L^o$ to get the facet embedding (i.e., sentence pattern embedding): $\underline{\vs}_{i,k} = L^o(\underline{\vd}_{i,k})$.
%paper embeddings are predicted using only one forward pass rather than using the autoregressive decoding as in~\citet{vaswani2017attention}. 






%adopt the cross attention

%There might be some dependency between 
%We use another 3-layer Transformer as our decoder to model the dependency of cluster centers as in~\citet{lee2018set}.

%We adopt the attention link between our encoder and decoder as in~\citet{vaswani2017attention} to avoid compressing all facets of the input text into one embedding $\underline{\vu}_{i,\text{\lessgreat{eos}}}$. 

%and the output embedding $\underline{\vb}_{i,k}$ is passed to our decoder $TD$: 
%\begin{align}




\subsection{Objective Function}
\label{sec:obj}

When measuring the distance between the $j$th entity pair and the $i$th sentence pattern, we compute the Euclidean distance between the entity pair embedding $\tilde{\underline{\ve}}_j$ and its closest facet embedding of the $i$th sentence pattern. The distance is defined as

\vspace{-3mm}
\small
\begin{align}
& D(\{\underline{\vs}_{i,k}\}_{k=1}^K, \tilde{\underline{\ve}}_j)  = \min_{k=1}^K \min_{0 \leq \eta_k \leq 1}|| \tilde{\underline{\ve}}_j - \eta_k \underline{\vs}_{i,k} ||^2,
\label{eq:dist_max}
\end{align}
\normalsize
\noindent where the entity pair embedding is normalized  (i.e., $||\tilde{\underline{\ve}}_j||=1$). During testing, we ignore the magnitude of facet embeddings, so we use $\eta_k$ to eliminate the magnitude of facet embeddings $\underline{\vs}_{i,k}$ during training. We do not allow negative $\eta_k$ to prevent the gradient flow from pushing $\underline{\vs}_{i,k}$ toward the inverse direction of $\tilde{\underline{\ve}}_j$ and we ensure $\eta_k \leq 1$ to avoid the neural model from outputting $\underline{\vs}_{i,k}$ with a very small magnitude. 


%prevent the neural model learning from outputting embedding that has an inverse direction of $\tilde{\underline{\ve}}_j$, and clamp $\eta_k$ below $1$ to prevent the output embedding from having a very small magnitude. 

As in Figure~\ref{fig:architecture}, we minimize the distance $D(\{\underline{\vs}_{i,k}\}_{k=1}^K, \tilde{\underline{\ve}}_j)$ in our loss function when the $i$th sentence pair co-occurs with the $j$th entity pair (i.e., $y_{i,j} = 1$). For negative samples (i.e., $y_{i,j} = 0$), we maximize the distance instead. That is, the major term of our loss function is defined as

\vspace{-3mm}
%\footnotesize
%\small
\begin{align}
& \sum_{(i,j) \in R} (2 \cdot y_{i,j}-1) r_{i,j}  D(\{\underline{\vs}_{i,k}\}_{k=1}^K, \tilde{\underline{\ve}}_j), 
\label{eq:dist_obj}
\end{align}
\normalsize
\noindent 
and the other regularization term $\Omega$ in the loss function will be described in \refAppendixAuto. $R$ is a set that includes all positive and negative samples. Positive samples are $(i,j)$ such that $y_{i,j} = 1$ and
the negative samples are constructed by pairing a randomly selected sentence pattern with the $j$th entity pair. %that co-occurs with the $i$th sentence pattern.
%of an sentence pattern are the entity pairs that co-occur with another randomly selected sentence pattern.
%where $\tilde{\underline{\ve}}_j$ is the normalized embedding of the $j$th entity pair where $||\tilde{\underline{\ve}}_j||=1$. 
%$r_{i,j}$
%negative samples: sample the entity pairs co-occurring with another sentence pattern
%For each positive sample $(i,j)$ such that $y_{i,j} = 1$, we create a negative sample by replacing the $i$th paper with a randomly selected paper. 
To balance the influence of popular entity pairs (i.e., entity pairs that co-occur with many sentence patterns) and rare entity pairs on our model,
%avoid the model biased toward the entity pairs that co-occur with many sentence patterns or relations,
%authors who write many papers, 
we set the weight of each pair, $r_{i,j} \propto \frac{1}{\sum_i {y_{i,j}}}$ and $\frac{\sum_{(i,j)\in R} r_{i,j}}{|R|} = 1$.
%normalize the weights to make the average of $r_{i,j}$ to be 1.

We generate the embeddings for KB relations in a similar way. We use a single token to represent the relation and append an \lessgreat{eos} (e.g., \emph{per:spouse} \lessgreat{eos}) to form the input of our neural model. 
%We suspect the KB relations need a larger number of embeddings because
The KB relations usually co-occur with more entity pairs, so we set the number of facet embeddings for KB relations $K_{rel}$ to be larger than the number of facet embeddings for sentence patterns $K$.

%For , 
%we treat KB relation the same (pass relation eos into the model)
%For KB relation, we use a different K




\subsection{Connection to Clustering}
\label{sec:cluster}

If a sentence pattern contains multiple facets that describe different relations between the entity pairs, the pattern often co-occurs with different kinds of entity pairs. For example, \textit{``\$ARG1 ’s partner \$ARG2''} in Figure~\ref{fig:architecture} could express the collaboration relationship between two companies or the partnership between two people, so the sentence patterns could co-occur with two companies such as \textit{(Google, Facebook)} and two people such as \textit{(Bob Bryan, Mike Bryan)}.

Different kinds of entity pairs often have very different embeddings, so we could discover the facets of sentence patterns by clustering the embeddings of entity pairs. Here, a facet refers to a mode of the embedding distribution of the entity pairs that could possibly co-occur with the sentence pattern. A facet could be represented by multiple facet embeddings and each facet embedding corresponds to a cluster center of the entity pair embeddings. Hence, although the number of facet embeddings $K$ is fixed for all the sentence patterns, our model can capture the facets of the sentence patterns well when the number of facets is less than $K$.


In \eqref{eq:dist_max}, we choose the closest facet embedding of the sentence pattern for each co-occurring entity pair embedding and minimize their distance. For example, $\underline{\vs}_{i,2}$ and the embedding of \textit{(Bob Bryan, Mike Bryan)} are pulled closer in Figure~\ref{fig:architecture}.
Minimizing \eqref{eq:dist_max} by passing the gradient through the scaled facet embedding $\eta_k \underline{\vs}_{i,k}$ is the same as minimizing a Kmeans loss, so the loss term induced by positive sample pairs encourage each $\underline{\vs}_{i,k}$ to become the cluster center of its nearby co-occurring entity pair embeddings. The details of our training algorithm could be found in \refAppendixMethod.

%For positive sample pairs
%, we are minimizing (1)
%explain directly using notation

The co-occurrence matrices in RE tasks are usually extremely sparse, and most of the sentence patterns only co-occur with a few entity pairs, which makes it difficult to derive multiple high-quality embeddings by clustering the co-occurring entity pair embeddings as in multi-sense word embedding %word sense induction 
methods such as~\citet{NeelakantanSPM14}. The proposed method solves this sparsity challenge by predicting the cluster centers using a neural model. For instance, even if \textit{``\$ARG1 's partner \$ARG2''} does not co-occur with many entity pairs, its embeddings are encouraged to be close to the embeddings of entity pairs that co-occur with other similar patterns (e.g., \textit{``\$ARG1 and her partner \$ARG2''}).

% Due to the continuity of neural network,
%of one sentence pattern (e.g., \textit{\$ARG1 's partner \$ARG2})
%the gradients from similar patterns such as \textit{\$ARG1 and his partner \$ARG2} will encourage the embeddings of \textit{\$ARG1 's partner \$ARG2}

%continuity of neural network will encourage the patterns with similar keywords to be similar \textit{\$ARG1 partner \$ARG2} or \textit{\$ARG1 and his partner \$ARG2}.


%challenge of learning multiple modes by clustering
%too sparse
%difficult to get high quality clusters by 
%directly cluster the 


%Sparsity challenge and why NN can aggregate the information from similar patterns
%using the figure as the example: even if \textit{\$ARG1 's partner \$ARG2} does not co-occur with lots of entity pairs, the continuity of neural network will encourage the patterns with similar keywords to be similar \textit{\$ARG1 partner \$ARG2} or \textit{\$ARG1 and his partner \$ARG2}.

%between $\tilde{\underline{\vs}}_{i,k}$ and $\tilde{\underline{\vs}}_{j,m}$

\begin{figure}[t!]
\centering
\includegraphics[width=1\linewidth]{fig/Scoring_function.pdf}
\caption{Comparison of the asymmetric similarities. $Asym(\{\tilde{\underline{\vs}}_{i,k}\},\{\tilde{\underline{\vs}}_{j,m}\} )>Asym(\{\tilde{\underline{\vs}}_{j,m}\},\{\tilde{\underline{\vs}}_{i,k}\} )$ because the average cosine distance on the left is smaller than that on the right.}
\label{fig:scoring}
\end{figure}

\subsection{Scoring Functions}
\label{sec:scoring}

In compositional universal schema, the similarity between the $i$th and $j$th sentence patterns are measured by the symmetric cosine similarity $\tilde{\underline{\vs}}^T_{i,1}   \tilde{\underline{\vs}}_{j,1}$, where $\tilde{\underline{\vs}}_{i,1} = \frac{\underline{\vs}_{i,1}}{||\underline{\vs}_{i,1}||}$. When using multiple embeddings to represent a sentence pattern, we can compute the asymmetric similarity as 

\vspace{-3mm}
%\footnotesize
\small
\begin{align}
&  Asym(\{\tilde{\underline{\vs}}_{i,k}\},\{\tilde{\underline{\vs}}_{j,m}\} ) = \frac{\sum_{m=1}^K \max\limits_{k=1}^K(  \tilde{\underline{\vs}}^T_{i,k}   \tilde{\underline{\vs}}_{j,m}  )}{K}.
\end{align}
\label{eq:asym_score}
\normalsize
\noindent In an example of Figure~\ref{fig:scoring}, a red square $\tilde{\underline{\vs}}_{i,k}$ is close to all the blue points, which leads to a high $Asym(\{\tilde{\underline{\vs}}_{i,k}\},\{\tilde{\underline{\vs}}_{j,m}\} )$.

Between two sentence patterns with entailment relation, we empirically find that the embeddings of a premise (the more specific pattern) often have some facet embeddings that are far away from all the embeddings of its hypothesis (the more general pattern). Relying on the tendency, we could detect the direction of the entailment relation. For example, the $i$th sentence pattern (red squares) in Figure~\ref{fig:scoring} is more likely to be premise if the $i$th and $j$th (blue circles) sentence patterns have an entailment relation. 

% for this tendency
We suspect the reason is that more specific patterns could contain more words that are similar to the words of other patterns expressing different relations.
%co-occurred with entity pairs with different relations. 
For example, \textit{``\$ARG1 , the wife of fellow \$ARG2''} have a facet embedding for spouse relation and another facet embedding for the co-worker relation because the pattern has high word overlapping with \textit{``\$ARG1 , the wife of \$ARG2''} and \textit{``\$ARG1 and her fellow \$ARG2''}. Another possible reason is that the articles in our corpus tend to use more specific patterns to express the relation between a pair of entities~\cite{shwartz2017hypernyms}.

%If $i$th and $j$th sentence patterns have a entailment relation and $Asym(\{\tilde{\underline{\vs}}_{i,k}\},\{\tilde{\underline{\vs}}_{j,m}\} )>Asym(\{\tilde{\underline{\vs}}_{j,m}\},\{\tilde{\underline{\vs}}_{i,k}\} )$, we can infer that $i$th sentence is more likely to be premise. 

%are often more diverse than

%(i,j)
%premise, hypothesis
%is similar to 

 

%model will predict the facets that are close to spouse when it sees spouse and close to co-worker when it sees fellow.

%specific could co-occur with more kinds of entity pairs
%Reversed Inclusion Measures


%To classify each sentence pattern
When performing RE, we compute the symmetric similarity between $i$th sentence pattern and $j$th KB relation $Sim(\{\tilde{\underline{\vs}}_{i,k}\},\{\tilde{\underline{\vs}}_{j,m}\} )$ by

\vspace{-3mm}
%\footnotesize
\small
\begin{align}
&  \frac{ Asym(\{\tilde{\underline{\vs}}_{i,k}\},\{\tilde{\underline{\vs}}_{j,m}\} ) + Asym(\{\tilde{\underline{\vs}}_{j,m}\}, \{\tilde{\underline{\vs}}_{i,k}\} ) }{2}.
\label{eq:sim_score}
\end{align}
\normalsize



%We use an example in Figure~\ref{fig:scoring} to illustrate the asymmetric similarity. One of the red 


%Sim
%Compare two sets of embeddings



%$D(\{\underline{\vs}_{i,k}\}_{k=1}^K, \tilde{\underline{\ve}}_j)$

%define reconstruct loss
%normalized sentence embedding
%asymmetric distance measurement


%need to explain why scoring function is like that (s2g > g2s). 

==> EACL 2021/content/method_details.tex <==
\label{sec:method_details}

%\section{Structure of Supplementary Materials}

Our objective function includes the loss defined in equation 2 and a regularization term $\Omega$. We describe $\Omega$ in Section~\ref{sec:auto} and some implementation details in Section~\ref{sec:implementation}. Finally, our training procedure is summarized in Algorithm~\ref{algo:dist_opt}.
%We first 

\subsection{Regularization by Autoencoder}
\label{sec:auto}

The co-occurrence matrix between the sentence patterns and entity pairs is very sparse because most of the sentence patterns only co-occur with a few entity pairs. The sparsity might make the training process of multi-facet embeddings sensitive to the hyperparameters. 

%between 1 and number of papers $I$
%significantly boost 
%the words in the sentence patterns are both input and output of our neural model. 


We discover that adding a simple autoencoder regularization is an effective way to stabilize the training. This regularization term aims to make the average of our facet embeddings of a sentence pattern similar to the weighted average of our word embeddings in that sentence pattern. The regularization is a kind of autoencoder because 
it reconstructs the weighted average embeddings of words in the input sentence pattern using the output facet embeddings.
The regularization term $\Omega$ is defined as 

\vspace{-3mm}
\small
\begin{align}
\gamma \sum_{ (i,j) \in R^{auto} } (2 \cdot \mathbbm{1}_{i=j}-1)|| \underline{\vs}^{aw'}_j - \mu(S_i) ||^2,
\label{eq:auto_dist}
\end{align}
\normalsize
where $\gamma$ is a weight for the regularization term, 
$R^{auto} = \cup_{i=1}^I \{(i,i),(i,q)\}$ is the set of all positive and negative training pairs, $I$ is the number of sentence patterns, and $q$ is a randomly selected index of sentence patterns which serves as our negative example, $\mathbbm{1}_{i=j} = 1$ if $i=j$ and $0$ otherwise, 
$\mu(S_i)= \frac{\sum_{k=1}^K \underline{\vs}_{i,k}}{K}$ is the average of facet embeddings of the sentence pattern $S_i$.
$\underline{\vs}^{aw'}_j$ is a weighted average embedding of words in the $j$th sentence pattern that passes through a linear transformation $\bm{H}$.
Weighting each word embedding by a smoothed inverse frequency provides a better text similarity measurement~\citep{arora2016simple} because the frequently occurring words often do not contribute much 
to the semantic meaning (e.g., stop words). Similarly
, we compute
\begin{align}
\underline{\vs}^{aw'}_j = \bm{H} \underline{\vs}^{aw}_j = \bm{H} \sum_{w \in S_j} \frac{\nu}{\nu + p(w)} \underline{\vw}, 
\label{eq:avg_word_emb}
\end{align}
where $\bm{H}$ linearly transforms 
the word embedding into the entity pair embedding space. $\nu=10^{-4}$ is a constant set suggested in \citet{arora2016simple}, $p(w)$ is the frequency of 
the word $w$ divided by the number of words in the corpus, and $\underline{\vw}$ is the pretrained embedding of word $w$. We use 840B GloVe~\cite{glove} as our word embedding in this work.


%\gamma
%, and $\gamma$ is a hyperparameters.
%, which will be defined in the next paragraph.
%play relatively less important roles in 
%to \citet{arora2016simple}
%a trainable matrix that linearly transforms
%probability of seeing the 

%We first compute a weighted average of word embeddings in each sentence pattern, project the average into the same space of entity pair embeddings, and encourage the average of our paper embeddings predicted by our neural model to be close to the average word embedding. 
%Most of the papers are only written by a few authors and cited by a few papers, so the interaction matrix is still very sparse even after jointly considering the authorship and citation information. If an author writes two papers and both papers are only cited by another paper, the papers are forced to have the same embedding even though the two papers have very different keywords in their titles and abstracts. This sparsity might encourage the embeddings of papers and authors in a small research subdomain to be collapsed into almost identical vectors.

%To learn more diverse paper embeddings (especially within small subdomains), 



%Since the words in the paper are both input and output of our neural model, the loss term $\Omega^{S}(F, \bm{H}, T)$ in 
%\refsimobj 
%is called autoencoder regularization. The autoencoder regularization is defined as 
%we call the regularization as autoencoder loss and define it as
% \small
% \begin{align}
%  \gamma \sum_{ (i,j) \in R^{auto} } \left( (\underline{\vp}^{aw'}_j)^T \mu(F(T_i)) - \mathbbm{1}_{i=j} \right)^2,
% \label{eq:auto}
% \end{align}
% \normalsize
% \noindent 



%Similarly to the loss of authorship and citation prediction, we modify the autoencoder regularization $\Omega^{D}(F, \bm{H}, T)$ function in 
%\refdistobj 
%\, as
%\begin{align}
%\gamma \sum_{ (i,j) \in R^{auto} } (2 \cdot \mathbbm{1}_{i=j}-1)|| \underline{\vp}^{aw'}_j - \mu(F(T_i)) ||^2,
%\label{eq:auto_dist}
%\end{align}


\begin{table}[t!]
\centering
\scalebox{0.9}{
\begin{tabular}{|c|c|c|}
\hline
Ours (Single-Trans) & Ours (Trans) & BERT Base \\ %\hline
1.0M & 1.1M & 86.0M \\ \hline 
Ours (Single-LSTM) & Ours (LSTM)  \\ %\cline{1-2}
2.6M & 3.0M \\ \cline{1-2}
\end{tabular}
}
\caption{Comparison of neural model sizes (i.e., the number of trainable parameters excluding the word embedding layer).}
\label{tb:model_size}
\end{table}


\begin{algorithm*}[!thp]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{Sentence patterns and KB relations $S$, co-occurrence matrix $\{y_{i,j}\}$, entity pair embeddings from USchema, and pre-trained word embeddings.}
\Output{Our neural encoder and decoder}
Initialize the entity pair embeddings using the embeddings learned by USchema. \\
Initialize the word embeddings of our neural encoder using pre-trained word embeddings and randomly initialize other parameters\\
\ForEach{$S_i$ \text{in training corpus}}{%
	Run forward pass on the neural encoder and decoder to compute facet embeddings $\{\underline{\vs}_{i,k}\}_{k=1}^K$ \\ % of sentence patterns
	Collect positive examples (i.e., $\{j|y_{i,j}=1\}$) and negative examples for the $i$th sentence pattern or KB relation\\
	\ForEach{\text{Positive and negative examples} $(i,j)$}{%
	Compute $\tilde{\underline{\ve}}_j= \frac{\underline{\ve}_j}{||\underline{\ve}_j||}$ \\
	Compute $\eta_k=\min(1,\max(0,\frac{\tilde{\underline{\ve}}^T_j \underline{\vs}_{i,k} }{||\underline{\vs}_{i,k}||^2})), \forall 1 \leq k \leq K$ \\
	Select $k_{best}$th facet embedding by $k_{best}=\argmin_{k} || \tilde{\underline{\ve}}_j - \eta_{k} \underline{\vs}_{i,k} ||^2$ \\
	Add $(2 \cdot y_{i,j}-1) r_{i,j} || \tilde{\underline{\ve}}_j - \eta_{k_{best}} \underline{\vs}_{i,k_{best}} ||^2$ to the loss
	}
	Add the autoencoder loss $\Omega$ in \eqref{eq:auto_dist} using pre-trained word embeddings\\
    Update neural encoder and decoder, entity pair embeddings, and $\bm{H}$ by backpropagation
}
 \caption{Training procedure (using batch size = 1)}
 \label{algo:dist_opt}
\end{algorithm*}

%Hyperparameter tuning methods
\subsection{Implementation Details}
\label{sec:implementation}

In our Transformer encoder and decoder, we set the number of layers to be 3 and the size of the hidden state to be 300. In our bi-LSTM encoder, the number of layers is set to 2. After the bi-LSTM encoder, we use the last embedding in the hidden state to encode a sequence into a single embedding. %as in \citet{verga2016multilingual}. 
In Table~\ref{tb:model_size}, we can see that the size of the neural model outputting multi-facet embeddings is similar to the size of the single embedding model, and both are much smaller than the BERT base model~\citep{BERT}. The size of CUSchema is smaller than ours because it uses a smaller hidden state size, but we find that increasing the model size of CUSchema does not lead to better performance.
%To make our method more comparable to CUSchema, we set 
%models, we set the 

%how many layers we have in Transformer and LSTM

%hidden state size is 300.

%2 layers

%bi-LSTM use max pooling to mimic Pat

Before training, we initialize the embeddings of entity pairs using USchema as in \citet{verga2016multilingual}. Besides, we initialize the word embedding layer in our neural model using GloVe. CUSchema initializes its word embedding layer randomly, but we also find that initializing it using pre-trained word embeddings does not increase the performance.

We use Adam~\cite{kingma2014adam} to optimize the parameters of our neural model and entity pair embeddings. For the linear layer $\bm{H}$ in \eqref{eq:avg_word_emb}, we adopt SGD to make the training more stable. Due to its small model size, one 1080Ti GPU is sufficient to train our model in 3 days.

%entity pair initialization like CUSchema, 
%We use 
%emphasize word embedding for Pat’s model is not useful
%Pat’s work has tuned the model size, so the improvement we get cannot be explained by the model size increase



==> EACL 2021/content/related_work.tex <==

Relation extraction (RE) is widely studied. \citet{han2020more} summarize the trend of recent studies and point out one of the major challenges is the cost of collecting the labels. Distant supervision~\citep{mintz2009distant} and its follow-up work enable us to collect a large amount of training data at a low cost, but the violation of its assumptions often introduces substantial noise into the supervision signal. Our goal is to alleviate the noise issue by representing every sentence pattern using multiple embeddings. 

Other noise reduction methods have also been proposed~\cite{roth2013survey}. For instance, we can adopt multi-instance learning techniques~\cite{yao2010collective, surdeanu2012multi,amin2020data}, global topic model~\cite{alfonseca2012pattern}, or both~\cite{roth2013feature}. We can also reduce the noise by counting the number of shared entity pairs between a sentence pattern and a KB relation~\cite{takamatsu2012reducing,su2018global}. Nevertheless, the studies focus on mitigating the noise caused by assuming similarity between the sentence patterns and KB relations that co-occur with the same entity pairs, while our method can also reduce the noise from two sentence patterns sharing the same entity pair. Besides, our method is complementary to popular noise reduction methods because our improvement is shown in the training data that have been cleaned~\citep{verga2016multilingual}.

%, %which assume that at least one of the sentence patterns 

%for a survey.
%RE Survey
%noise reduction

%At least one \cite{yao2010collective}
%multi-instance learning (At least one)\cite{yao2010collective, surdeanu2012multi,amin2020data}

%topic model\cite{alfonseca2012pattern}

%Hybrid: At least one assumption and global topic statistics 
%\cite{roth2013feature}

%pattern correlation 


%What’s the difference between our method and other noise removal methods

%all the denoising methods focus on KB relations, and our method could be applied to unsupervised relation discovery?

Our method is conceptually related to some studies for lexical semantics. For example, word sense induction or unsupervised hypernymy detection can be addressed by clustering the co-occurring words~\citep{NeelakantanSPM14,athiwaratkun2017multimodal,chang2018distributional}. However, the clustering-based methods do not apply to RE because the co-occurring matrix for RE is much sparser (see Section~\ref{sec:cluster} for more details).

%ir method is designed to 
%and is not applicable to RE.  
%In universal schema, the relation co-occurring matrix is much sparser than word co-occurring matrix used in \citet{NSD} and 
%we propose novel techniques to overcome the challenge such as an autoencoder regularization,

Finally, our work is inspired by 
\citet{NSD}, but they focus on improving the sentence representation rather than RE. We encourage the facet embeddings to become the centers in Kmeans clustering instead of NNSC (non-negative sparse coding) clustering used in \citet{NSD}, due to its simplicity, efficiency, and better RE performance. Moreover, we discover that an additional regularization described in \refAppendixAuto is crucial to overcome the sparsity challenge in RE. 
%for our multi-facet model
%Moreover, 
%because Kmeans loss is simpler and more efficient, and also leads to better RE performances.


%Their loss encourages the sentence embeddings to become the cluster centers 
% by predicting  cluster centers

%predicting 
%sparsity issue

%hypernym
%\cite{shwartz2017hypernyms}
%\cite{chang2018distributional}
%global clustering

%Not applicable to RE. 
%Kmeans loss is much faster than NNSC loss used in \citet{NSD}, and Kmeans seems to also achieve the better results in RE.




%We discover that Kmeans seem to be better than NNSC in \citet{NSD} and being faster works similarly with Kmeans, but Kmeans is faster

%We use Kmeans clustering rather than NNSC clustering



==> EACL 2021/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

